Entropy Is Not Enough: Unlocking Effective Reinforcement Learning for Visual Reasoning via Vision-Anchored Token Selection

While token-level entropy is commonly recognized as effective for credit assignment in text-only reinforcement learning with verifiable rewards (RLVR), it remains unclear whether this mechanism still holds in visual reasoning. Our controlled study shows that this mechanism collapses in visual reasoning due to the omission of vision-sensitive tokens with naturally low entropy. Although existing multimodal RL methods increasingly acknowledge the importance of visual perception, they struggle to satisfy the inherent demand for interleaving precise perceptual grounding with semantic reasoning, either lacking systematic visual measurements or overlooking that token entropy primarily drives semantic exploration. To address this, we introduce VEPO (Vision-Entropy token-selection for Policy Optimization), an effective RL framework explicitly integrating visual sensitivity with token entropy via a principled multiplicative coupling, where VEPO redirects gradient credit toward tokens which are simultaneously visually grounded and highly informative. Extensive experiments demonstrate VEPO's leading performance, significantly outperforming the entropy-only baseline by 2.28 points at 7B-scale and 3.15 points at 3B-scale. Ablations further substantiate the soundness of our method.

==> Table/table_ablation_hyperparameters.tex <==
\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{8pt}
\begin{tabular}{c|ccccc}
\toprule
$k$ / $\alpha$& 0.1 & 0.3 & 0.5 & 0.7 & 0.9 \\
\midrule
0.2 & 56.51 & 56.92 & 57.36 & \textbf{58.80} & 57.53 \\
0.3 & 56.39 & \underline{58.28} & 58.14 & 57.99 & 56.85 \\
0.4 & 55.74 & 55.77 & 55.97 & 57.38 & 56.27 \\
\bottomrule
\end{tabular}
\caption{Ablation on the balancing coefficient $\alpha$ and the token retention ratio $k$. The best result is shown in bold and the second-best result is underlined.}
\label{tab:ablation_alpha_k}
\end{table}

